Spotting Suspicious Link Behavior with fBox: An Adversarial Perspective

How can we detect suspicious users in large online networks? Online popularity of a user or product (via follows, page-likes, etc.) can be monetized on the premise of higher ad click-through rates or increased sales. Web services and social networks which incentivize popularity thus suffer from a major problem of fake connections from link fraudsters looking to make a quick buck. Typical methods of catching this suspicious behavior use spectral techniques to spot large groups of often blatantly fraudulent (but sometimes honest) users. However, small-scale, stealthy attacks may go unnoticed due to the nature of low-rank eigenanalysis used in practice. In this work, we take an adversarial approach to find and prove claims about the weaknesses of modern, state-of-the-art spectral methods and propose fBox, an algorithm designed to catch small-scale, stealth attacks that slip below the radar. Our algorithm has the following desirable properties: (a) it has theoretical underpinnings, (b) it is shown to be highly effective on real data and (c) it is scalable (linear on the input size). We evaluate fBox on a large, public 41.7 million node, 1.5 billion edge who-follows-whom social graph from Twitter in 2010 and with high precision identify many suspicious accounts which have persisted without suspension even to this day.

==> 040problem.tex <==
In this paper we aim to further restrict the size of attacks available to
spammers.  Formally, we define the following problem:


\begin{problem}
	Given an adjacency matrix $G$ of honest users, define an algorithm that
	limits the number of edges that can be add by $n$ spammers pointing to $m$
	users without being caught.
\end{problem}


==> 070related.tex <==
%%\subsection{Anomaly Detection} % (fold)
%%\label{par:Anomaly detection}

{\noindent \bf Anomaly detection:}
%% Anomaly detection is another well-studied field and is closely related to other
%% contexts such as fraud identification and intrusion detection.
%%\cite{aggarwal2001outlier} details the poor
%%performance of traditional distance metrics for identifying anomalies in sparse
%%high-dimensional spaces and proposes outlier detection methods on
%%low-dimensional projections. 
%\cite{ghosh2012understanding} proposes an approach penalizing promiscuous users on Twitter, but is only shown to be effective in detecting already caught spammers rather than detecting new ones. 
%\cite{shrivastava2008mining} and \cite{ying2011spectrum} use graph topology to tackle a similar problem of detecting Random Link Attacks (RLA) with sparsely connected victim nodes --- such an assumption does not hold in our case. 
%\cite{berkeleyspam} focuses on malicious Tweets and finds that blacklisting approaches are too slow to stem the spread of Twitter spam.  
%\cite{netprobe07pandit} uses belief propagation to find near-bipartite cores of attackers on eBay. 
%\cite{malspot14} uses tensor decomposition to detect network intrusions.  
%\cite{eigenspokes10} and \cite{jiang14} are two notable spectral approaches further detailed in Section~\ref{sec:background}. 

%%\subsection{Community Detection} % (fold)
%%\label{par:Community detection}
{\noindent \bf Community detection:}
%% There has been an extensive amount of work in the field of mining communities
%% and clusters in social graphs.  Graph partitioning is one popular approach for
%% studying connectivity structure in graph data.  In this context,
%\cite{ng2001spectralA} and \cite{huang2008spectral} propose using eigenvectors
%of graph decompositions for partitioning. 
\cite{metis} and \cite{graclus} focus on cut-based metrics for partitioning, but perform poorly on sparse social graphs lacking good cuts.  
\cite{kcore11} and \cite{dcore11} propose 
%% means of quantifying
methods of measuring the
cooperation and collaboration in communities 
in undirected and directed graphs.   

%\subsection{Adversarial Analysis} % (fold)
%\label{par:Adversarial analysis}

{\noindent \bf Adversarial analysis:}
%% Several works have been conducted in the context of motivating improved
%% detection algorithms via adversarial analysis.  
%\cite{domingoskdd04} and \cite{lowd2005adversarial} propose game theoretic approach between spam classifiers and omniscient adversaries and demonstrate weaknesses of linear classifiers on email spam.
%%\cite{liu2009game} and \cite{bruckner2012static} model adversarial learning in
%%terms of Stackelberg and Nash coordination games.  
%\cite{cobafi} proposes a collaborative filtering
%model that limits the impact of spam by clustering users.
However, much of the prior work in adversarial analysis is primarily focused on
text rather than graph-based learning.



 %\cite{shrivastava2008mining} - random walk based for RLAs


==> FIG-TIKZ/block.tex <==
\begin{tikzpicture}[scale=0.4]
\pgfmathsetseed{2}
\draw (0,0) rectangle (10,10);
\filldraw[fill=red!12] (7,0) rectangle (10,3);
\fillrandomly{0}{3}{7}{10}{0.03}{200}{black}
%\fillrandomly{7}{0}{10}{3}{0.01}{1000}{red}

   \node[black, font=\small] at (-2.0,1.5)                    {Fraudsters};
   \node[black, font=\small] at (-2.0,6.5)                    {Real fans};

   \draw[<->,black] (-0.3,0) -- (-0.3,2.99) ;
   \draw[<->,black] (-0.3,3.01) -- (-0.3,10);


   \draw[<->, black] (0,-0.3) -- (6.98,-0.3) ;
   \draw[<->, black] (7.02,-0.3) -- (10,-0.3);
   \node[black, font=\small] at (3.5,-0.8)                    {Honest accounts};
   \node[black, font=\small] at (8.5,-0.8)                    {Customers};

\end{tikzpicture}


==> FIG-TIKZ/camo.tex <==

\begin{tikzpicture}[scale=0.4]
   \coordinate (A) at ( 0, 0);
   \coordinate (topleft) at (0,10);
   \coordinate (bottomright) at (10,0);
   \coordinate (B)  at (10,10);
   \coordinate (X)  at (3,5);
   \coordinate (XX) at (3,0); % x-value of crossing, to help with calculations
   \coordinate (XY) at (0,5); % y-value of crossing, to help with calculations
   \coordinate (L)  at (-1,0); % 'Left' margin, for the arrows
   \coordinate (F)  at (0,-1); % 'Floor' margin, for the arrows

   % \draw [style=help lines] (A) grid (B);
   \draw [thin] (A) rectangle (B);
   % \draw [fill=green!5]  (0,0) rectangle (8,7);
   % \node at (A) [rectangle,fill=gray]  {camo};
   % \draw [fill=gray!15]  (0,0) rectangle (7,2);
   % \node at (0,5) [rectangle,draw] {attack};
   \draw [fill=gray!5] (A) rectangle (X);
   % \node at (1.5,2.5)                    {camo};
   \node at ($1/2*(A) + 1/2*(X)$)          {camo};
   
   \draw [fill=gray!15] (X) rectangle (topleft);
   \node at ($1/2*(X) + 1/2*(topleft)$)   {normal};
   
   \draw [fill=gray!70]   (X)  rectangle (bottomright);
   \node at ($1/2*(X) + 1/2*(bottomright)$)  {attack};
   
   
   \node at (4,3)     [circle,fill=white,draw]  {} ;
   \node at (5.5,1.5) [circle,fill=white,draw]  {} ;
   
   \draw [<->] (L) -- ($(L) + (XY)$);

   % \draw [<->] (-1,5) -- (-1,10) ;
   \draw [<->] ($(L) + (XY)$) -- ($(L) + (topleft)$);

   % christos will substitute all 'magic numbers' with parms
   \node at (-3, 2.5)                   {botnet};
   \node at (-3, 7.5)                   {honest fans};
   
   \draw[<->] (0,-1) -- (3,-1) ;
   \draw[<->] (3,-1) -- (10,-1);
   \node at (1.5,-2)                    {honest idols};
   \node at (7.5,-2)                    {'customers'};

\end{tikzpicture}


==> FIG-TIKZ/random.tex <==
\begin{tikzpicture}[scale=0.4]
\pgfmathsetseed{2}
\draw (0,0) rectangle (10,10);
\fillrandomly{0}{3}{7}{10}{0.03}{200}{black}
\fillrandomly{7}{0}{10}{3}{0.03}{1000}{red!60}

   \node[black, font=\small] at (-2.0,1.5)                    {Fraudsters};
   \node[black, font=\small] at (-2.0,6.5)                    {Real fans};

   \draw[<->,black] (-0.3,0) -- (-0.3,2.99) ;
   \draw[<->,black] (-0.3,3.01) -- (-0.3,10);


   \draw[<->, black] (0,-0.3) -- (6.98,-0.3) ;
   \draw[<->, black] (7.02,-0.3) -- (10,-0.3);
   \node[black, font=\small] at (3.5,-0.8)                    {Honest accounts};
   \node[black, font=\small] at (8.5,-0.8)                    {Customers};

\end{tikzpicture}


==> FIG-TIKZ/staircase.tex <==
\begin{tikzpicture}[scale=0.4]
\pgfmathsetseed{2}
\draw (0,0) rectangle (10,10);

%\filldraw[fill=red!12] (7,2) rectangle (9,3);
%\filldraw[fill=red!12] (8,1) rectangle (10,2);
%\filldraw[fill=red!12] (9,0) rectangle (10,1);
%\filldraw[fill=red!12] (7,0) rectangle (8,1);

\fill[fill=red!12] (7,2.25) rectangle (8.5,3);
\fill[fill=red!12] (7.75,1.5) rectangle (9.25,2.25);
\fill[fill=red!12] (8.5,0.75) rectangle (10,1.5);
\fill[fill=red!12] (9.25,0) rectangle (10,0.75);
\fill[fill=red!12] (7,0) rectangle (7.75,0.75);

\draw (7,0) rectangle (10,3);

\fillrandomly{0}{3}{7}{10}{0.03}{200}{black}

   \node[black, font=\small] at (-2.0,1.5)                    {Fraudsters};
   \node[black, font=\small] at (-2.0,6.5)                    {Real fans};

   \draw[<->,black] (-0.3,0) -- (-0.3,2.99) ;
   \draw[<->,black] (-0.3,3.01) -- (-0.3,10);


   \draw[<->, black] (0,-0.3) -- (6.98,-0.3) ;
   \draw[<->, black] (7.02,-0.3) -- (10,-0.3);
   \node[black, font=\small] at (3.5,-0.8)                    {Honest accounts};
   \node[black, font=\small] at (8.5,-0.8)                    {Customers};

\end{tikzpicture}


==> makefile <==
MAIN= paper
FINAL= final
TEXPARTS= 			\
    000abstract.tex 		\
    010introduction.tex 	\
    015background.tex		\
    020adversarial.tex		\
    030bigpic.tex		\
    040problem.tex		\
    050algo.tex			\
    060conclusions-gplus.tex	\
    060experiments.tex		\
    070related.tex		\
    080conclusion.tex		\
    090appendix.tex		\
    dfn.tex



BIBPARTS= BIB/*.bib
FIGTIKZPARTS= FIG-TIKZ/*.pdf FIG-TIKZ/*.tex 
FIGPARTS= figs/* figs/*/*
# FIG/*.png FIG/*.dia $(FIGTIKZPARTS)
STYPARTS= sig-alternate.cls
OTHER= mkfinal.pl makefile 
ALL= $(MAIN).tex $(TEXPARTS) $(BIBPARTS) $(FIGPARTS) \
     $(FIGTIKZPARTS) $(STYPARTS) $(OTHER)

# $(FIGTIKZPARTS)
$(MAIN).pdf: $(MAIN).tex $(TEXPARTS)  
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

final: $(FINAL).pdf

# $(FIGTIKZPARTS)
$(FINAL).pdf: $(MAIN).tex mkfinal.pl $(TEXPARTS)  
	mkfinal.pl $(MAIN).tex > $(FINAL).tex
	pdflatex $(FINAL).tex
	bibtex $(FINAL)
	pdflatex $(FINAL).tex
	pdflatex $(FINAL).tex

try: $(MAIN).tex
	pdflatex $(MAIN)


clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak *.lbl *.brf
	\rm -f *.out

spotless: clean
	\rm -f $(MAIN).ps $(MAIN).pdf
	\rm -f $(FINAL).*
	\rm -rf TST

all.tar:
	tar cvfh all.tar $(ALL)

pccite: 2014-icdm-pc.txt
	grep "^\*\*\*" 2014-icdm-pc.txt 

